Symbolic Knowledge Distillation: from General Language Models to Commonsense Models

The common practice for training commonsense models has gone from-human-to-corpus-to-machine: humans author commonsense knowledge graphs in order to train commonsense models. In this work, we investigate an alternative, from-machine-to-corpus-to-machine: general language models author these commonsense knowledge graphs to train commonsense models. Our study leads to a new framework, Symbolic Knowledge Distillation. As with prior art in Knowledge Distillation (Hinton et al., 2015), our approach uses larger models to teach smaller models. A key difference is that we distill knowledge symbolically-as text-in addition to the neural model. We also distill only one aspect-the commonsense of a general language model teacher, allowing the student to be a different type, a commonsense model. Altogether, we show that careful prompt engineering and a separately trained critic model allow us to selectively distill high-quality causal commonsense from GPT-3, a general language model. Empirical results demonstrate that, for the first time, a human-authored commonsense knowledge graph is surpassed by our automatically distilled variant in all three criteria: quantity, quality, and diversity. In addition, it results in a neural commonsense model that surpasses the teacher model's commonsense capabilities despite its 100x smaller size. We apply this to the ATOMIC resource, and share our new symbolic knowledge graph and commonsense models.

==> figures/fig_head_tail_counts.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/head_tail_counts.png}
    \caption{Unique heads $|(\cdot,\texttt{relation},\texttt{tail})|$ and unique tails $|(\texttt{head},\texttt{relation},\cdot)|$
    for the  \automic\ and \atomic\ knowledge bases.
    }
    \label{fig:head-tail-counts}
\end{figure}

==> figures/fig_tsne.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/tsne_full_half.pdf}
    \caption{Visual comparison of \automic\ and \atomic\ data.
    Each point represents a (head, relation, tail) encoded with RoBERTa and embedded with T-SNE.
    Points from \automic\ are shown with `x' and colored by datasource, with numbered kmeans clusters. \autotomic shows high overlap with \atomic while both show novel clusters of generations (e.g. 4, 10, 26).
    % Unique heads $|(\cdot,\texttt{relation},\texttt{tail})|$ and unique tails $|(\texttt{head},\texttt{relation},\cdot)|$
    % for the  \automic\ and \atomic\ knowledge bases.
    }
    \label{fig:tsne-main}
\end{figure}

==> figures/fig_tsne_app.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/tsne_full.pdf}
    \caption{Visual comparison of \automic\ and \atomic\ data.
    Each point represents a (head, relation, tail) encoded with RoBERTa and embedded with T-SNE.
    Points from \automic\ are shown with `x'. Right: colored by datasource, with numbered kmeans clusters. Left: colored by relation. 
    % Unique heads $|(\cdot,\texttt{relation},\texttt{tail})|$ and unique tails $|(\texttt{head},\texttt{relation},\cdot)|$
    % for the  \automic\ and \atomic\ knowledge bases.
    }
    \label{fig:tsne}
\end{figure*}

==> figures/fig_unique_tails.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/unique_tails.png}
    \caption{Unique tails (inferences) by relation.}
    \label{fig:unique-tails}
\end{figure}

==> figures/per_relation_tsne.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_HinderedBy-crop.pdf}
    \caption{T-SNE plot on examples with the HinderedBy relation
    }
    \label{fig:tsne_HinderedBy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xAttr-crop.pdf}
    \caption{T-SNE plot on examples with the xAttr relation
    }
    \label{fig:tsne_xAttr}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xEffect-crop.pdf}
    \caption{T-SNE plot on examples with the xEffect relation
    }
    \label{fig:tsne_xEffect}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xIntent-crop.pdf}
    \caption{T-SNE plot on examples with the xIntent relation
    }
    \label{fig:tsne_xIntent}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xNeed-crop.pdf}
    \caption{T-SNE plot on examples with the xNeed relation
    }
    \label{fig:tsne_xNeed}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xReact-crop.pdf}
    \caption{T-SNE plot on examples with the xReact relation
    }
    \label{fig:tsne_xReact}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/per_relation_tsne/tsne_xWant-crop.pdf}
    \caption{T-SNE plot on examples with the xWant relation
    }
    \label{fig:tsne_xWant}
\end{figure}



==> sections/3_purification_0.tex <==
\section{Making the Teacher More Critical}
\label{sec:purification}


While the \emph{loose teacher} (GPT-3 alone) results in a viable commonsense knowledge graph, human evaluation suggests this isn't a perfect commonsense teacher.
Thus, we multiply in a \emph{critic model}, to filter out lower-quality knowledge, thereby \emph{correcting the teacher} (\S\ref{subsec:knowledgedistillation}). With a modest amount of supervision in the form of a small-scale human evaluation, we can train a classifier to predict and discriminate unacceptable examples. We multiply this with the \emph{loose teacher} \S\ref{sec:verbalization}, creating a \emph{critical teacher} product of experts. In practice this means filtering the generations in \autotomic and creating a range of new corpora that are higher quality, yet still larger scale than \atomic. %Surprisingly, automatic models trained on human evaluation can discriminate unacceptable examples \emph{very effectively}, resulting in purified corpora that are both high quality and larger scale than human. Here, we describe this process, and its application to \autotomic.

%to leverage the very large scale from verbalization to greatly increase CSKB accuracy. 

% In this section, we describe the process of purification (\S\ref{subsec:purification}), and demonstrate its effect on the quality of \autotomic (\S\ref{subsec:purificationeval})

%\subsection{Purifying a Generated CSKB}
\label{subsec:purification}

% \subsubsection{Human Supervision}
%Purification requires human supervision, in the form of small-scale evaluation for tuning a model.
We first gather a training set of \textit{correct vs. incorrect} human judgments on a randomly-sampled set of 10K entries of \autotomic.  We follow the evaluation from \S~\ref{subsec:atomichuman}, but gather one annotation per example. We take a (random) train/dev/test split of 8k/1k/1k. While this aspect of \skd is not entirely automatic, this evaluation is similar in cost/complexity to other evaluations in the paper, and much cheaper/easier than elliciting human-authored knowledge. Rather, humans become high-level supervisors.


We train binary classifiers (critics) for human acceptability using RoBERTa-Large \cite{liu2019roberta}. We find pretraining on MNLI results in the best precision/recall model, and suggest this for future work. We give more detail in Appendix~\ref{app:critic}, including baselines. Our best model vastly improves the accuracy of \autotomic (Table~\ref{tbl:ATOMIC-human}), demonstrating that a small amount of human supervision can consistently help to correct GPT-3's mistakes. 

\paragraph{Size-accuracy Trade-off} As with any filtration process, our critic faces a trade-off between size and accuracy based on what cutoff is used. We offer several versions of \autotomic representing different cutoffs, i.e. the confidence at which the critic rejects an example. We report human-measured accuracy (Accept/Reject column Table~\ref{tbl:ATOMIC-human}) following \S\ref{subsec:atomichuman}.
By discarding the 20\% of the instances the classifier judges as least acceptable (reducing knowledge graph size from 6.5M to 5.1M)
%Yet comparing to human-generated \atomic tells us the trade-off is favorable.
%By reducing size from 6.5M to 5.1M (approx. 20\% reduction),
\autotomic's accuracy rises from 78.5 $\rightarrow$ 88.4; human-authored \atomic contains only 600K entries at 86.8\% accuracy. Reducing to 2.5M examples (38\% of the original size), we can attain an accuracy of 96.4\%, nearly 10 points above the human \corpus. To put this in perspective, at this cutoff, \autotomic is still 4X larger than \atomic.

% One takeaway is that scale is a strong advantage of automatic knowledge generation: attempting a similar filtering step on human-generated \atomic would further reduce its already smaller size. 

%\paragraph{Does Human Acceptability Improve Across Cutoffs?}


% The goal of purification is raising the quality of our generated \corpus, \autotomic. By human evaluation (Table~\ref{tbl:COMET-human}--\S\ref{subsec:verbalization-eval}) we can see that this is successful. The top row of \autotomic--without purification--has a human acceptance rate of 78.5\%. Even under our lowest threshold for purification (second row of), this rises to 88.4\% acceptance, exceeding the human-generated \atomic. Our highest setting increases this to 96.4\%, a full 17.9 points above the unpurified \corpus. A small amount of human supervisions results in a highly effective purifier.


%\subsection{The Effect of Purification on Diversity}
\label{subsec:purificationeval}



\paragraph{What gets filtered out?}

We qualitatively identify two types of filtered triples: 1) \emph{logical misalignments}, which consist of events/inferences joined in a logically inconsistent manner. Identification of these triples requires modeling logical interactions between events and inferences, e.g., \textit{X cannot find his shirt \textbf{as a result X} is wearing a shirt}, \textit{X was kidnapped \textbf{as a result X feels} safe}.; and 2) \emph{awkward phrasings}, which consist of events/inferences that, in isolation, are incoherent, ambiguous, or awkwardly phrased. Examples of events with awkward phrasings that were include: \textit{PersonX has a fire in the bath} and \textit{PersonX appears to be three-dimensional}; any inference that completes these events may be unacceptable because the event itself is broadly implausible.

\input{tables/purify_ablation}
To understand what types of triples are filtered (and in what frequency), we ablate our critic model: the validation precision-recall results, summarized by average precision (AP), are given in Table~\ref{tbl:purification_ablation}: our full model is compared to a random predictor, a event-only model, and a inference-only model, all based on RoBERTa. We also compare to an additive EMAP \cite{hessel2020emap} version of our model that computes an optimal additive ensemble of event-only and inference-only models, but doesn't allow for logical interactions between the event/inference to be incorporated (as would be required to identify \emph{logical misalignments}).

We find that GPT-3 produces both independently awkwardly-phrased events/inferences and also logical misalignments. But, our classifier, trained on validated knowledge triples, helps in both cases. The EMAP of our full model (which can identify only awkward phrasings) achieves 87\% AP, and our full model (which can additionally identify logical misalignments) improves performance to 94\% AP.

%make the distinction between these two GPT-3 failure cases concrete, we say that an awkwardly phrased $(\texttt{\textbf{h}ead},\texttt{\textbf{r}elation}, \texttt{\textbf{t}ail}) = (h,r,t)$ triple is one that


\paragraph{Does Filtering Hurt Diversity?}
%Besides raising accuracy, how does purification affect \autotomic? One attribute we are particularly interested in diversity--
One concern is the critic reducing \autotomic to only similar ``safe'' examples that may not be novel in practice. We repeat our diversity analysis from \S\ref{subsec:verbalization-eval} for the various cutoffs; results are in Table~\ref{tbl:ATOMIC-human} (``Size (div)'', higher=better). As we filter more stringently, we surprisingly observe proportionally \emph{more} diverse examples:
% we are filtering some diverse examples \jack{can we put something in here about the proportionality?}. This gives no indication that the relative diversity of the \corpus goes down:
full \autotomic has a diverse subset  68\% of its size; this goes up to 80\% for the most filtered version. GPT-3 may possibly gravitate towards common sentence structures which represent inconsistent knowledge. These would be highly recognizable to the critic, and removing them would increase both quality and diversity. This surprising result warrants further study.

% Yet diversity and human-judged quality do not tell the whole story. We are not only interested in intrinsic measures--but rather how \textit{useful} a generated CSKB will be in practice. To study this, we move onto distillation \S\ref{sec:distillation}, where we measure how effective each \corpus is for training the downstream commonsense model.

==> sections/backups/0_introduction_0.tex <==
\section{Introduction}
\label{sec:intro}
\input{figures/fig_1}

Commonsense Knowledge Bases (CSKBs) \cite{hwang2020comet,sap2019atomic,speer2017conceptnet} are a critical source for \textit{the kinds of information we expect most humans to know}. They are central to research with commonsense \cite{chakrabarty-etal-2020-r, ammanabrolu2020automated, Kearns2020AWI, chakrabarty2021mermaid}, providing trustworthy and interpretable information for model reasoning \cite{Zhang2020ASERAL} and training \cite{Bosselut2019COMETCT}. Naturally, CSKBs are usually constructed by humans, with a common recipe going \textit{human-to-corpus-to-model}: humans write examples of commonsense at a large scale--the CSKB--and this knowledge is used to train downstream commonsense models. Yet, the high cost and complexity of human annotation makes this paradigm difficult to apply and scale; simultaneously, the recent human-like knowledge of large language models (LMs) \citep{gpt3} suggests an alternative paradigm, replacing \textit{human} with \textit{model}.

To explore this possibility, we propose \textbf{\skd}, going \textit{model-to-corpus-to-model}. Our method parallels knowledge distillation \cite{Hinton2015KnowledgeDistill}; in that method and ours, a larger teacher model transfers knowledge to a more compact and usable student model--we find the underlying objectives of the methods highly related (\S\ref{subsec:knowledgedistillation}). Yet an important difference we find is that our method results in a student that \emph{surpasses} the teacher--the opposite is often true in knowledge distillation (cite). \Skd also functions differently: while model distillation transfers knowledge directly through gradient updates, our knowledge takes a natural language form first. This allows us to choose \textit{which} knowledge is transferred, allowing us to distill only some aspects--the commonsense knowledge--from the general teacher model. This also means that, besides the student model, a large CSKB is a natural product of our method.

\SKD Works in 3 steps, beginning with a source model--GTP-3--and ending in a more compact commonsense model. First is \textbf{verbalization}: GPT-3 generates a large scale of natural commonsense knowledge, using few-shot learning. This results in an initial corpus. The second step, \textbf{purification}, takes advantage of the interpretable form this knowledge takes. Training a discriminator on human judgements, we find the corpus can be filtered to very high accuracy while retaining a large scale. Finally, in \textbf{distillation} a downstream commonsense model is trained on the corpus. The resulting model is smaller, more efficient, and produces commonsense at a higher accuracy than the teacher--GPT-3. 

Besides comparing our commonsense model to its teacher, we are interested in how this paradigm compares to the human-driven, \textit{human-to-corpus-to-model} paradigm. We take a recent instance of this--\citet{hwang2020comet}, in which humans author \atomicorig-style \citep{sap2019atomic} data (\atomic), and compare this to \skd. We find our machine-generated corpus (\autotomic) can exceed the human generated corpus in scale, accuracy, and diversity. The resulting commonsense model--\model in our case--also surpasses the human-trained equivalent--\comet. Indeed, \skd offers a promising path to bypass the need for human-authored commonsense; this opens possibilities for larger and less expensive datasets, better commonsense models, as well as the rapid acceleration and expansion of commonsense research that these will allow.

==> sections/backups/0_introduction_1_peter.tex <==
\section{Introduction}
\label{sec:intro}
\input{figures/fig_1}

Commonsense Knowledge Bases (CSKBs) \cite{hwang2020comet,sap2019atomic,speer2017conceptnet} are central to research involving model understanding \cite{chakrabarty-etal-2020-r, ammanabrolu2020automated, Kearns2020AWI, chakrabarty2021mermaid}, providing trustworthy and interpretable information for model training \cite{Bosselut2019COMETCT} and reasoning \cite{Zhang2020ASERAL}. CSKBs enumerate many examples of commonsense, \textit{the kind of information we expect most humans to know}. Naturally, CSKBs are often constructed by humans, particularly for complex information. A common recipe goes \textit{human-to-\corpus-to-model}: humans author a \corpus of commonsense examples at a large scale--the CSKB--and this knowledge is used to train downstream commonsense models (CITE EXAMPLES). Yet, the high cost and complexity of human annotation makes this paradigm difficult to apply and scale. Simultaneously, the recent human-like knowledge of large language models (LMs) \citep{gpt3} suggests an alternative paradigm, replacing \textit{human} with \textit{model}.

To explore this possibility, we propose \textbf{\skd}, going \textit{model-to-\corpus-to-model}. Our method parallels knowledge distillation \cite{Hinton2015KnowledgeDistill}: in that method and ours, a larger teacher model transfers knowledge to a more compact and usable student model--we find the underlying objectives of the methods highly related (\S\ref{subsec:knowledgedistillation}). Yet an important difference we find is that our method results in a student that \emph{surpasses} the teacher. The opposite is often true in knowledge distillation (CITE). \Skd also functions differently: while knowledge distillation transfers knowledge directly through gradient updates, our knowledge takes an intermediate, natural language form. This allows us to choose \textit{which} knowledge is transferred, and thus distill only some aspects--high quality commonsense--from the general teacher model. This also means that, along with the student model, a large CSKB is a natural product of our method.

\SKD Works in 3 steps, beginning with a source model--GTP-3--and ending in a more compact commonsense model. First is \textbf{verbalization}: GPT-3 generates a large scale of natural commonsense knowledge, using few-shot learning. This results in an initial \corpus. The second step, \textbf{purification}, takes advantage of the interpretable form this knowledge takes. Training a discriminator on human judgements, we find the \corpus can be filtered to very high accuracy while retaining a large scale. Finally, in \textbf{distillation} a downstream commonsense model is trained on the \corpus. The resulting model is smaller, more efficient, and produces commonsense at a higher accuracy than the teacher--GPT-3. 

To compare to the human-driven, \textit{human-to-\corpus-to-model} paradigm, we take a recent instance of this--\citet{hwang2020comet}, in which humans author \atomicorig-style \citep{sap2019atomic} data (\atomic), and we compare this to \skd. We find our machine-generated \corpus (\textbf{\autotomic}) exceeds the human generated \corpus in scale, accuracy, and diversity. The resulting commonsense model--\textbf{\model}--also surpasses the human-trained equivalent--\comet. Indeed, \skd offers a promising path to bypass the need for human-authored commonsense; this opens possibilities for larger and less expensive datasets, better commonsense models, as well as the rapid acceleration and expansion of commonsense research that these will allow.

==> sections/backups/1_introduction_1_jack.tex <==
\section{Introduction}
\label{sec:intro}
\input{figures/fig_1}

Commonsense Knowledge Bases (CSKBs) \cite{hwang2020comet,sap2019atomic,speer2017conceptnet} have proven to be an effective means of teaching models basic facts about how the world works \cite{chakrabarty-etal-2020-r, ammanabrolu2020automated, Kearns2020AWI, chakrabarty2021mermaid, Bosselut2019COMETCT, Zhang2020ASERAL}. Broadly speaking, these KBs enumerate many examples of otherwise unstated background information about the physical, causal, and social worlds that are known to most humans (e.g., \jack{example}). 
% While most humans know these types of facts as second nature, they may be difficult (or impossible) for models to learn without being explicitly told.

%These resources have proven instrumental  , providing trustworthy and interpretable information for model training \cite{Bosselut2019COMETCT} and reasoning \cite{Zhang2020ASERAL}. These KBs , and, 

%\textit{the kind of information we expect most humans to know}

Naturally, CSKBs are typically constructed by humans. A common recipe is \textit{human-to-\corpus-to-model}: humans author a large collection of commonsense examples, forming the CSKB, and this knowledge is used to train downstream  models (CITE EXAMPLES). Yet, the high cost and complexity of human annotation makes this paradigm difficult to apply and scale. And, recent work in large language models (LMs) \citep{gpt3} trained without structured knowledge suggests that significant (but incomplete) commonsense information can indeed be learned directly from web data; thus human annotation efforts risk duplicating information that models can already represent effectively.

We propose an alternative paradigm: replacing \textit{human} CSKB authors with a \textit{language model}. Specifically, we propose \textbf{\skd}, that goes \textit{model-to-\corpus-to-model}. Our method parallels usual knowledge distillation \cite{Hinton2015KnowledgeDistill} in that a larger teacher model transfers knowledge to a more compact and usable student model.
%--we find the underlying objectives of the methods highly related (\S\ref{subsec:knowledgedistillation}).
Yet an important difference is that the knowledge is compressed in a human-readable (and editable) \emph{symbolic} format (rather than less-interpretable model logits, as in standard KD). This representation enables precise interventions on what knowledge is transferred: we can interpretably correct the mistakes the general teacher model (GPT-3) makes, and distill only high quality commonsense to the student. In the end, we are left with not only a large, high-quality CSKB, but also a distilled student model that \emph{surpasses} its teacher.
%The opposite is often true in knowledge distillation (CITE).
%\Skd also functions differently: while knowledge distillation transfers knowledge directly through gradient updates, our knowledge takes an intermediate, natural language form.
% This allows us to choose \textit{which} knowledge is transferred, and thus distill only some aspects--high quality commonsense--from the general teacher model.
%This also means that, along with the student model, a large CSKB is a natural product of our method.

\SKD works in 3 steps.
%beginning with a source model--GPT-3--and ending in a more compact commonsense model.
First is \textbf{verbalization} (\S\ref{sec:verbalization}): GPT-3 generates a large scale of commonsense knowledge via few-shot learning; this results in an initial natural language \corpus. The second step, \textbf{purification} (\S\ref{sec:purification}), takes advantage of the interpretable knowledge format: by training a discriminator on a comparatively small set of human judgements, we identify the teacher model's mistakes, and filter the \corpus to very high accuracy while maintaining large scale. Finally, in \textbf{distillation} (\S\ref{sec:distillation}), a downstream commonsense model is trained on the \corpus. To compare \skd against the \textit{human-to-\corpus-to-model} paradigm, we consider \citet{hwang2020comet}, in which humans author \atomicorig-style \citep{sap2019atomic} data (\atomic). We find our machine-generated \corpus, \textbf{\autotomic}, exceeds the human generated \corpus in scale, accuracy, and diversity. The resulting commonsense model, \textbf{\model}, not only surpasses the human-trained equivalent \comet, but is also smaller, more efficient, and produces commonsense at a higher accuracy than the teacher--GPT-3. 

\Skd offers a promising path for more effective model and human collaboration. Our work demonstrates that humans and LMs can be effective collaborators for curating CSKBs and training efficient+performant commonsense models. \textbf{We release XYZ}
%\jack{I do like this story of compromise... I wonder if we can end on the "humans and machines have different strengths" story?} 
%By bypassing the need for fully human-authored commonsense this opens possibilities for larger and less expensive datasets, better commonsense models, as well as the rapid acceleration and expansion of commonsense research that these will allow.

==> sections/backups/1_overview_0.tex <==
\section{Overview and Background}
\label{sec:overview}

We describe the \textit{model-to-corpus-to-model} paradigm of \skd in 3 steps. First, \textit{model-to-corpus}: we call this \textbf{verbalization} (\S\ref{sec:verbalization}). A very large language model--GPT-3--is used to \textit{generate} commonsense data; a large-scale machine-generated commonsense knowledge base (CSKB), the \textit{corpus}, is the result. 

Next, we describe the \textbf{purification} step (\S\ref{sec:purification}), going corpus-to-corpus. Human evaluation can tell us which generated examples are high quality knowledge. A discriminator trained on these human judgements can tell us this as well, with surprising effectiveness. In the purification step, we use this discriminator to filter down our generated CSKB, to high human-judged quality. 

Finally, we cover \textit{corpus-to-model}, the \textbf{distillation} step (\S\ref{sec:distillation}). A compact, efficient commonsense model is trained on our corpus--in effect, the knowledge extracted from GPT-3 is transferred into a purified, compact, and usable form. 

The \textit{model-to-corpus-to-model} form of \skd parallels that of knowledge distillation \cite{Hinton2015KnowledgeDistill}; both transfer knowledge from a large and ``cumbersome'' model to a compact and usable one. Indeed, both methods optimize a similar objective, with key differences due to the \textit{generation} step of \skd.

\subsection{Knowledge Distillation by Generating}
\label{subsec:knowledgedistillation}

Knowledge distillation was introduced by \citet{Hinton2015KnowledgeDistill}, to transfer the learned knowledge from a ``cumbersome'' or difficult to use distribution $P_t$ (e.g. an ensemble of models) to a more usable usable form $P_s$ (e.g. a single model). For instance, the teacher $P_t$ may be an ensemble of large speech recognition experts, whose knowledge is \textit{distilled} into a simpler student model $P_s$. 

A key aspect of distillation is matching the probabilities of $P_s$ to $P_t$, encouraging the student to have a similar distribution; this is how knowledge is transferred. In its simplest form\footnote{specifically, setting the softmax temperature $T=1$. Temperature is useful for controlling the learning signal but less principled in theory.}, we want to minimize the distance--cross entropy--between $P_t$ and $P_s$ for each input example:

$$ H(P_t,P_s) = \sum_{v \in Y} P_t(v)logP_s(v)$$

\noindent
where $Y$ is the set of labels. By minimizing this, we are encouraging $P_s$ to mimic $P_t$. We are particularly interested in generative models here though, where possible outputs are the infinite set of strings $S$. One proposed extension to knowledge distillation in this setting is to use the teacher to smooth labels of token-level cross entropy \cite{Sanh2019DistilBERTAD}. Specifically, when learning to continue partial string $x$, we can smooth word labels with $P_t$ rather than just taking ground truth $y$:

$$ L(P_t,P_s) =  \sum_{v \in Y} P_t(v|x)logP_s(v|x)$$

\noindent
One issue with this approach is that it does not represent a principled generative notion: partial sequence $x$ comes from a training distribution $X$, sampled form a \textit{different} distribution than $P_t$, although $P_t$ may be learned to mimic it. \citet{Kim2016SequenceLevelKD} propose to treat the set of possible sequences as labels from \citet{Hinton2015KnowledgeDistill}; this results in a principled notion of cross entropy, learning $P_s$ to mimic $P_t$:

$$ H(P_t,P_s) = \sum_{s \in S} P_t(s)logP_s(s)$$

\noindent
In practice, it is impossible to enumerate $S$. \citet{Kim2016SequenceLevelKD} roughly approximate this objective by collapsing onto the mode, although this is not guaranteed to be a good estimate. An alternative approach giving a true estimate of this cross entropy would be to \textit{sample} from $P_t$:

$$ H(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim P_t} logP_s(s)$$

\noindent
\Skd is based on this formulation. One particular advantage of sampling is that it gives us fine control over what \textit{aspects} of $P_t$ we would like to distill into $P_s$. In this work, we use GPT-3 as the teacher $P_t$, a vast and general model. We can apply deliberate constraints $c$ to what kinds of samples to to take from $P_t$:

$$ L_{SKD} =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim c(P_t)} logP_s(s)$$

\noindent
For instance, we one aspect of constraint set $c$ is that we only sample knowledge related to specific notions of commonsense (\S\ref{sec:verbalization}). Another is that we constrain these samples to meet learned notion of quality (\S\ref{sec:purification}). These ensure that, by the time the knowledge is distilled into a final model $P_s$ (\S\ref{sec:distillation}), it contains only the target information. This particular notion of selectively distilling information of a general model, through text, is the central idea of \skd.


$$ H(P_t,P_s) \approx \frac{1}{n} \sum_{i=1}^{n}\sum_{v \in V} P($$

Our work follows a similar formulation to knowledge distillation \cite{Hinton2015KnowledgeDistill}, but with key differences which we outline here.
Knowledge distillation works by compressing a teacher distribution $P_t$ into a more compact or usable student distribution $P_s$. $P_t$ may be an ensemble of models \cite{Hinton2015KnowledgeDistill} or a very large model (cite distilbert, something in vision). For example, distilBERT (cite distilbert) compresses a full-size BERT model into a smaller and more efficient version of the same model. Knowledge distillation was originally posed to minimize a distance (cross entropy $H$ cite) between $P_t$ and $P_s$ on an existing dataset. Supposing the teacher $P_t$ captures the underlying data distribution well, this is roughly given as:

$$ H(P_t,P_s) \approx \frac{1}{n}\sum_{x_i \in X}\sum_{w \in V} P_t(w|x)logP_s(w|x)$$

\noindent
where $V$ is the set of labels and $x$ is an input example in the dataset  $X$. This often contains other terms, including temperature and gold label matching, with the stated goal of matching $P_t$. $P_s$ is thus trained to capture the same knowledge as $P_t$, by mimicking the soft labels of $P_t$, $P_t(w|x)$, rather than ground truth $y$ \peter{Think about the gold label aux loss}. In the generative setting, we can capture this same distance with sampling:

$$ H(p||q) \propto lim_{n\xrightarrow{}\infty}\frac{1}{n}\sum_{x \sim P_t} log(P_s(x))$$

\noindent
Rather than transferring knowledge about $P_t$ through soft labels on existing data, sampling captures this knowledge in a symbolic form. This is the basis of symbolic knowledge distillation. While it sacrifices the dense learning signal of soft labels, it has other benefits--especially allowing more control over this learning signal. 

\peter{Cite \citet{Kim2016SequenceLevelKD}. SPECIFICALLY in terms of ``SKD allows us to control the distribution. One simple way is to truncate low-quality elements of the distribution, using top-p which is shown to be more effective at this than beam search used in Kim and Rush.''}


We can explicitly constrain sampling to capture only the type of knowledge we would like to distill. This can mean sampling only in a specific domain (e.g. commonsense knowledge), sampling only high-probability outputs, or even removing sampled outputs that are deemed to be incorrect--a level of control not possible with the continuous learning signal in knowledge distillation. Constrained sampling gives us a new objective function $S_c$: 

$$S_c(P_t||P_s) = lim_{n \xrightarrow{} \infty{}}\frac{1}{n}\sum_{x \sim c(P_t)} log(P_s(x))$$

\noindent
where $c$ is a set of constraints applied to sampling. In the simplest form where there are no constraints $c$, this simplifies to KL divergence between $P_t$ and $P_s$, optimizing the same objective as vanilla knowledge decoding. In this work however, we explore how this sampling can be constrained to distill specific and high quality knowledge in the commonsense knowledge domain.
\peter{maybe bring up why we don't compare to KD: (i) GPT-3 distribution is not fully available, just 100 logits, and (ii) KD relies on static data to transfer on. If we use arbitrary data, may not transfer domain-specific knowledge. If we use domain data (ATOMIC) then we are using human data which is cheating. Also bring up the `no logits needed' idea as a specific benefit of SKD}

\subsection{Data: \atomicorig}
\label{subsec:atomicdata}

As we describe \skd, we demonstrate it on the \atomicorig \textit{if-then} corpus \cite{sap2019atomic}: Our verablization and purificaiton result in a new corpus--\autotomic. The distillation step produces a commonsense model--\model, much like past work using \atomicorig \cite{Bosselut2019COMETCT,hwang2020comet}. Throughout the process, we compare the resources we generate with comparable and state-of-the-art human-generated equivalent--\atomic and \comet. 

\atomicorig follows an event-relation-tail format. A large set of \textit{events} forms the foundation of the corpus, e.g. \textit{X attacks Y}. An \atomicorig example links a relation to an event, like the \textbf{HinderedBy} relation which describes something that might hinder this event. For a given relation and head, the goal is to generate a resulting tail generation, e.g. \textit{X attacks Y} \textbf{HinderedBy} \textit{X is restrained}. 

Of the 23 relations from the most recent CSKB--\atomic--we limit our investigation to 7: \textbf{xAttr} (how X is perceived after \textit{event}), \textbf{xReact} (how X reacts in response to \textit{event}), \textbf{xEffect} (what X does after \textit{event}), \textbf{xIntent} (X's intent in \textit{event}), \textbf{xWant} (what X wants after \textit{event}), \textbf{xNeed} (what X needed for \textit{event}) and \textbf{HinderedBy}. 

==> sections/backups/1_overview_1.tex <==
\section{Overview and Background}
\label{sec:overview}

We describe the \textit{model-to-corpus-to-model} paradigm of \skd in 3 steps. First, \textit{model-to-corpus}: we call this \textbf{verbalization} (\S\ref{sec:verbalization}). A very large language model--GPT-3--is used to \textit{generate} commonsense data; a large-scale machine-generated commonsense knowledge base (CSKB), the \textit{corpus}, is the result. 

Next, we describe the \textbf{purification} step (\S\ref{sec:purification}), going corpus-to-corpus. Human evaluation can tell us which generated examples are high quality knowledge. A discriminator trained on these human judgements can tell us this as well, with surprising effectiveness. In the purification step, we use this discriminator to filter down our generated CSKB, to high human-judged quality. 

Finally, we cover \textit{corpus-to-model}, the \textbf{distillation} step (\S\ref{sec:distillation}). A compact, efficient commonsense model is trained on our corpus--in effect, the knowledge extracted from GPT-3 is transferred into a purified, compact, and usable form. 

The \textit{model-to-corpus-to-model} format of \skd parallels that of knowledge distillation \cite{Hinton2015KnowledgeDistill}; both transfer knowledge from a large and ``cumbersome'' model to a compact and usable one. Indeed, these methods optimize a similar objective, a key difference being  \textit{generation} step of \skd.

\subsection{Knowledge Distillation by Generating}
\label{subsec:knowledgedistillation}

Knowledge distillation was introduced by \citet{Hinton2015KnowledgeDistill}, to transfer the learned knowledge from a ``cumbersome'' or difficult to use distribution $P_t$ (e.g. an ensemble of models) to a more usable usable form $P_s$ (e.g. a single model). For instance, the teacher $P_t$ may be an ensemble of large speech recognition experts, whose knowledge is \textit{distilled} into a simpler student model $P_s$. 

A key aspect of distillation is matching the probabilities of $P_s$ to $P_t$, encouraging the student to have a similar distribution; this is how knowledge is transferred. In its simplest form\footnote{specifically, setting the softmax temperature $T=1$. Temperature is useful for controlling the learning signal but less principled in theory.}, we want to minimize the distance--cross entropy--between $P_t$ and $P_s$ for each input example:

$$ H(P_t,P_s) = \sum_{v \in Y} P_t(v)logP_s(v)$$

\noindent
where $Y$ is the set of labels. By minimizing this, we are encouraging $P_s$ to mimic $P_t$. We are particularly interested in generative models here though, where possible outputs are the infinite set of strings $S$. One proposed extension to knowledge distillation in this setting is to use the teacher to smooth labels of token-level cross entropy \cite{Sanh2019DistilBERTAD}. Specifically, when learning to continue partial string $x$, we can smooth word labels over vocabulary $V$ with $P_t$ rather than just taking ground truth $y$:

$$ L(P_t,P_s) =  \sum_{v \in V} P_t(v|x)logP_s(v|x)$$

\noindent
One potential issue with this approach is a mismatch between data and soft labels: partial sequence $x$ comes from a training set $X$, sampled form a \textit{different} distribution than $P_t$, although $P_t$ may be learned to mimic it. \citet{Kim2016SequenceLevelKD} propose instead to think of \textit{full sequences} as the labels; this results in a principled notion of cross entropy, learning $P_s$ to mimic $P_t$ over the set of all possible labels (strings) $S$:

$$ H(P_t,P_s) = \sum_{s \in S} P_t(s)logP_s(s)$$

\noindent
In practice, it is impossible to enumerate $S$. \citet{Kim2016SequenceLevelKD} roughly approximate this objective by collapsing onto the mode, although this likely misses a lot of information from $P_t$\footnote{In their work, \citet{Kim2016SequenceLevelKD} specifically note the mode covers a single-digit percentage of the full distribution}. An alternative approach covering more of $P_t$ would be to \textit{sample} from $P_t$:

$$ H(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim P_t} logP_s(s)$$

\noindent
\Skd is based on this formulation. Sampling naturally leverages the frequentist notion of distribution $P_t$ as a data generator: sampling a very large corpus from $P_t$ will come to represent the distribution fully, as sample size grows. Any information we could learn from $P_t$ will eventually appear in the sampled data.  

One particular advantage of sampling is that it gives us fine control over what \textit{aspects} of $P_t$ we would like to distill into $P_s$. In this work, we use GPT-3 as the teacher $P_t$, a vast and general model. We can apply deliberate constraints $c$ to what kinds of samples to take from $P_t$:

$$ L_{SKD} =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim c(P_t)} logP_s(s)$$

\noindent
For instance, in our experiments, one aspect of constraint set $c$ is that we only sample knowledge related to specific notions of commonsense (\S\ref{sec:verbalization}). Another is that we constrain these samples to meet a learned notion of quality (\S\ref{sec:purification}). These ensure that, by the time the knowledge is distilled into a final model $P_s$ (\S\ref{sec:distillation}), it contains only the desired information. In a sense, we are not over-burdening student $P_s$ with learning irrelevant aspects of $P_t$ (GPT-3). This particular notion of selectively distilling information of a general model, through text, is the central idea of \skd.

\subsection{Data: \atomicorig}
\label{subsec:atomicdata}

As we describe \skd, we demonstrate it on the \atomicorig \textit{if-then} corpus \cite{sap2019atomic}: Our verablization and purificaiton result in a new corpus--\autotomic. The distillation step produces a commonsense model--\model, much like past work using \atomicorig \cite{Bosselut2019COMETCT,hwang2020comet}. Throughout the process, we compare the resources we generate with comparable and state-of-the-art human-generated equivalent--\atomic and \comet. 

\atomicorig follows an event-relation-tail format. A large set of \textit{events} forms the foundation of the corpus, e.g. \textit{X attacks Y}. An \atomicorig example links a relation to an event, like the \textbf{HinderedBy} relation which describes something that might hinder this event. For a given relation and head, the goal is to generate a resulting tail generation, e.g. \textit{X attacks Y} \textbf{HinderedBy} \textit{X is restrained}. 

Of the 23 relations from the most recent CSKB--\atomic--we limit our investigation to 7: \textbf{xAttr} (how X is perceived after \textit{event}), \textbf{xReact} (how X reacts in response to \textit{event}), \textbf{xEffect} (what X does after \textit{event}), \textbf{xIntent} (X's intent in \textit{event}), \textbf{xWant} (what X wants after \textit{event}), \textbf{xNeed} (what X needed for \textit{event}) and \textbf{HinderedBy}. 

==> sections/backups/1_overview_2.tex <==
\section{Overview and Background}
\label{sec:overview}

Throughout our work, we describe the \textit{model-to-corpus-to-model} process of \skd, continuously comparing to the \textit{human-to-corpus-to-model} alternative \cite{hwang2020comet}. We devote 1 section to each of the 3 steps of \skd. 

We describe the \textit{model-to-corpus-to-model} paradigm of \skd in 3 sections, one for each step. First, \textit{model-to-corpus}: we call this \textbf{verbalization} (\S\ref{sec:verbalization}). A very large language model--GPT-3--is used to \textit{generate} commonsense data; a large-scale machine-generated commonsense knowledge base (CSKB), the \textit{corpus}, is the result. 

Next, we describe the \textbf{purification} step (\S\ref{sec:purification}), going corpus-to-corpus. Human evaluation can tell us which generated examples are high quality knowledge. A discriminator trained on these human judgements can tell us this as well, with surprising effectiveness. In the purification step, we use this discriminator to filter down our generated CSKB, to high human-judged quality. 

Finally, we cover \textit{corpus-to-model}, the \textbf{distillation} step (\S\ref{sec:distillation}). A compact, efficient commonsense model is trained on our corpus--in effect, the knowledge extracted from GPT-3 is transferred into a purified, compact, and usable form. 

The \textit{model-to-corpus-to-model} format of \skd parallels that of knowledge distillation \cite{Hinton2015KnowledgeDistill}; both transfer knowledge from a large and ``cumbersome'' model to a compact and usable one. Indeed, these methods optimize a similar objective, a key difference being  \textit{generation} step of \skd.

\subsection{Knowledge Distillation by Generating}
\label{subsec:knowledgedistillation}

Knowledge distillation was introduced by \citet{Hinton2015KnowledgeDistill}, to transfer the learned knowledge from a ``cumbersome'' or difficult to use distribution $P_t$ to a more usable usable form $P_s$. For instance, the teacher $P_t$ may be an ensemble of large speech recognition experts, whose knowledge is \textit{distilled} into a simple student model $P_s$. This framing is a natural fit for extracting knowledge from GPT-3, a large and effective, yet inaccessible model.

A key aspect of distillation is matching the probabilities of $P_s$ to $P_t$, encouraging the student to have a similar distribution; this is how knowledge is transferred. In its simplest form\footnote{specifically, setting the softmax temperature $T=1$. Temperature is useful for controlling the learning signal but less principled in theory.}, we want to minimize the distance--cross entropy--between $P_t$ and $P_s$ for each input example:

\begin{equation}
    H(P_t,P_s) = \sum_{v \in Y} P_t(v)logP_s(v)
    \label{eq:kd}
\end{equation} 

\noindent
where $Y$ is the set of labels. By minimizing this, we are encouraging $P_s$ to mimic $P_t$. In this work, we are interested in transferring knowledge \textit{generatively}, such that the student model can \textit{author} commonsense knowledge. One natural way to do this is introducing these soft labels to the language modelling objective \cite{Sanh2019DistilBERTAD} for generation:

\begin{equation}
    L(P_t,P_s) =  \sum_{i=0}^{len(x)} \sum_{v \in V} P_t(v|x_{1:i})logP_s(v|x_{1:i})
    \label{eq:Ldistilbert}
\end{equation} 

\noindent
when learning on example sequence $x$, over vocabulary $V$. In effect, replacing the gold word labels of cross entropy loss with soft labels from the teacher, GPT-3. This has a number of issues, first and foremost the full distribution of soft labels is not currently accessible\footnote{At the time of writing, the API for GPT-3 only returns up to the top 100 token probabilities, out of thousands.}. There is also an intrinsic mismatch with this objective: the soft labels of $P_t$ come from a different distribution than the underlying data $x$. Perhaps most importantly, we may not want to distill \textit{all knowledge} from GPT-3 uniformly. GPT-3 contains a vast quantity of knowledge, much of which may be irrelevant--in this work we are only interested in its commonsense. While we can control the data $x$ in Eq~\ref{eq:Ldistilbert}, we cannot control what information is transferred through soft labels, which will result in wasted training signal and student model capacity.

In fact, we can alleviate all of these issues by simply reframing the knowledge distillation objective (Eq~\ref{eq:kd}) for generation. Rather than distilling at the token level, we can do this at the sequence level:

\begin{equation}
    H(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim P_t} logP_s(s)
    \label{eq:seqCE}
\end{equation}

\noindent
In effect, information about $P_t$ is captured by the frequentist notion of \textit{which full sequences it samples}, rather than its soft labels. \citet{Kim2016SequenceLevelKD} follow a similar formulation, but represent the distribution with the mode alone rather than samples. This framing alleviates the need for access to the full distribution, and removes the mismatch between data and soft labels--indeed, it now captures the principled notion of cross entropy. Most important, we now have precise control over what information is transferred, through what information is \textit{sampled}. \Skd works by applying constraints $c$ to this sampling:

\begin{equation}
    L_{SKD}(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim c(P_t)} logP_s(s)
    \label{eq:seqCE}
\end{equation}

\noindent
For instance, in our experiments, one aspect of constraint set $c$ is that we only sample knowledge related to specific notions of commonsense (verbalization \S\ref{sec:verbalization}). Another is that we constrain these samples to meet a learned notion of quality (purification \S\ref{sec:purification}). These ensure that, by the time the knowledge is distilled into a final model $P_s$ (\S\ref{sec:distillation}), it contains only the desired information. In a sense, we are not over-burdening student $P_s$ with learning irrelevant aspects of $P_t$ (GPT-3). This particular notion of distilling specific information from a general model, through text, is the central idea of \skd.



\subsection{Data: \atomicorig}
\label{subsec:atomicdata}

As we describe \skd, we demonstrate it on the \atomicorig \textit{if-then} corpus \cite{sap2019atomic}: Our verablization and purificaiton result in a new corpus--\autotomic. The distillation step produces a commonsense model--\model, much like past work using \atomicorig \cite{Bosselut2019COMETCT,hwang2020comet}. To understand how machine knowledge differs from human, we compare our resources with state-of-the-art equivalents--\atomic and \comet. 

\atomicorig follows an event-relation-tail format. A large set of \textit{events} forms the foundation of the corpus, e.g. \textit{X attacks Y}. An \atomicorig example links a relation to an event, like the \textbf{HinderedBy} relation which describes something that might hinder this event. For a given relation and head, the goal is to generate a resulting tail generation, e.g. \textit{X attacks Y} \textbf{HinderedBy} \textit{X is restrained}. 

Of the 23 relations from the most recent CSKB--\atomic--we limit our investigation to 7: \textbf{xAttr} (how X is perceived after \textit{event}), \textbf{xReact} (how X reacts in response to \textit{event}), \textbf{xEffect} (what X does after \textit{event}), \textbf{xIntent} (X's intent in \textit{event}), \textbf{xWant} (what X wants after \textit{event}), \textbf{xNeed} (what X needed for \textit{event}) and \textbf{HinderedBy}. 

==> sections/backups/1_overview_3.tex <==
\section{Overview and Background}
\label{sec:overview}

Throughout our work, we describe the \textit{model-to-corpus-to-model} methodology of \skd, with model-to-corpus verbalization (\S\ref{sec:verbalization}), corpus to corpus purification (\S\ref{sec:purification}), and corpus to model distillation (\S\ref{sec:distillation}). Throughout, we contrast it with the \textit{human}-driven alternative \cite{hwang2020comet}

\Skd naturally follows the large-to-small model compression of knowledge distillation \citep{Hinton2015KnowledgeDistill}, yet our use of generated knowledge results in a fundamentally different process.

\subsection{Knowledge Distillation by Generating}
\label{subsec:knowledgedistillation}

Our proposed methodology parallels knowledge distillation (KD) \cite{Hinton2015KnowledgeDistill}, a method for
% The original motivation for KD was to
compressing a large teacher model into a smaller student model with as little performance degradation as possible. 
In our work, the teacher is GPT-3 \cite{gpt3}, a 175-billion parameter language model.
% may be an ensemble of large speech recognition experts, whose knowledge is \textit{distilled} into a single student model $P_s$.
%, used here, is naturally a ``cumbersome'' model.

%both transfer knowledge from a large and ``cumbersome'' model to a compact and usable one. 

% While these methods optimize a similar objective, yet a key difference is \textit{generation} in \skd.

% This closely mirrors a section in the intro already.
% We devote 1 section to each of the 3 steps of \skd. First, \textit{model-to-\corpus}: we call this \textbf{verbalization} (\S\ref{sec:verbalization}). A large language model--GPT-3--\textit{generates} commonsense data; a large-scale generated CSKB is the result. Second, the \textbf{purification} step (\S\ref{sec:purification}), going \corpus-to-\corpus. Human evaluation tells us which generations are high quality; a discriminator trained on these human judgements does so as well, with surprising effectiveness. Here, we use this discriminator to filter down our CSKB, to high human-judged quality. Finally, going \textit{\corpus-to-model}, the \textbf{distillation} step (\S\ref{sec:distillation}). An efficient commonsense model is trained on our \corpus--the knowledge extracted from GPT-3. 
%\subsection{Knowledge Distillation by Generating}
%\label{subsec:knowledgedistillation}



%Knowledge distillation was introduced by \citet{Hinton2015KnowledgeDistill}, to transfer the learned knowledge from a ``cumbersome'' or

Traditional knowledge distillation transfers knowledge to a student model $P_S$ by optimizing the student so that its outputs match those of a teacher $P_t$.
% parameters of $P_s$ 
% KD's training objective fixes the parameters of $P_t$, and optimizes $P_s$ 
% to match the teacher's outputs. 
For language modeling, this means optimizing the parameters of $P_s$ to  minimize the cross entropy on each input sequence $x$:
% between a 
% For discrete distributions, this means minimizing the cross entropy between $P_t$ and $P_s$ for each input example $x$,
%\footnote{Softmax temperature $T=1$. Temperature is useful for controlling the learning signal but less principled in theory.},
% \begin{equation}
%     H(P_t,P_s,x) = -\sum_{v \in V} P_t(x)_v \log P_s(x)_v,
%     \label{eq:kd}
% \end{equation} 
% \noindent
% where $V$ is a vocabulary. % , such that the student model can \textit{author} commonsense.
% In language modeling, the distillation objective for a sequence $x$ is:
$L(P_s;P_t,x) =$% Distil-GPT , given a 
% A natural way to do this is by introducing these soft labels to the language modelling objective for generation \footnote{distilGPT uses this method.}:
\begin{equation}
    -\sum_{i=1}^{|x|} \sum_{v \in V} P_t(x_i|x_{<i})_v\log P_s(x_{i}|x_{<i})_v.
    \label{eq:Ldistilbert}
\end{equation} 

\noindent
Instead of transferring knowledge via per-token probabilities, we are interested in transferring knowledge through natural language,
% . Natural language is a more appealing interface for our setting, 
% as it enables a controllable interface for knowledge curation, letting 
as it enables us to edit, filter, and constrain the knowledge that is transferred. % (\S \ref{sec:purification}).
% , this enables ; and 2) we may not be interested in $P_s$ matching the distribution of $P_t$ for \emph{all} possible inputs --- for example, in this work, we are only interested in GPT-3's commonsense.
% (and not, say, it's \jack{something bad here like... IDK, dark reddit comments or something}).
%

To this end, we develop a \textit{sampled sequence distillation} objective that operates on discrete sequences sampled from a constrained teacher $P_t^*$,
\begin{equation}
    L_{\mathrm{SKD}}(P_s; P_t) =  \mathop{\mathbb{E}}_{x \sim P^*_t(x)}[-\log P_s(x)].
    \label{eq:seqCE}
\end{equation}
\noindent
Operating on sequences enables knowledge transfer through natural language, while the constrained teacher $P_t^*$ -- formally, a distribution whose support is a subset of the original teacher's $P_t$ -- offers control over the transferred knowledge.
For instance, an auxiliary model $A(x)$ can accept or reject sequences, $P^*_t(x) \propto P_t(x)\cdot A(x)$, which enables flexibly incorporating human feedback (\S\ref{sec:purification}).
The objective corresponds to minimizing sequence-level cross-entropy, enabling controlled, natural language knowledge transfer in a principled way.

% we reformulate the language modeling KD objective (Eq~\ref{eq:Ldistilbert}) in two ways: 1) to enable a natural language interface, we operate on sampled sequences from $P_t$; and 2) we sample sequences $x$ from a constrained portion of the teacher distribution we are interested in reconstructing $P^*_t(x)$, rather than the full distribution $P_t(x)$. 
% The constraints we utilize are flexible. For example, prompt $p$ can specify the teacher distribution via $P^*_t(x) = P_t(x|p)$ (\S\ref{sec:verbalization}); and, an acceptability estimation model $A(x)$ an be directly for purification, i.e., $P^*_t(x) \propto P_t(x|p)\cdot A(x)$ (\S\ref{sec:purification}). For whichever curation is selected, for a constrained teacher $P^*_t(x)$, we optimize student using the \emph{sampled distillation} LM loss:

%Rather than distilling at the token level (Eq~\ref{eq:Ldistilbert}), we do this at the sequence level:
%In effect, replacing the gold word labels of the cross entropy with soft labels from $P_t$.
%However, in our work this is GPT-3, for which this distribution of soft labels is not currently available\footnote{At the time of writing, the API for GPT-3 only returns up to the top 100 token probabilities, out of thousands.}.
%There is also an intrinsic mismatch in this objective: the soft labels of $P_t$ come from a different distribution than the underlying data $x$.
%Most importantly, we do not want to distill \textit{all knowledge} from GPT-3 uniformly. GPT-3 contains a vast quantity of knowledge, and much is irrelevant--in this work we are only interested in its commonsense. We can imagine controlling this through the training data $x$ in Eq~\ref{eq:Ldistilbert}, yet we cannot control what is transferred through soft labels.

% \begin{equation}
%     L_{SKD}(P_t,P_s) =  \mathop{\mathbb{E}}_{x \sim P^*_t(x)}[-logP_s(x)]
%     \label{eq:seqCE}
% \end{equation}

% \noindent
% In effect, information about $P^*_t$ is captured by the frequentist notion of \textit{which full sequences $x$ it samples}, rather than soft word labels. 
% 
% \citet{Kim2016SequenceLevelKD} use a similar sequence-level formulation, but use only the mode from an unconstrained teacher.
% 
% rather than sample from distribution. 
% Operating on sequences enables knowledge transfer through natural language, and only requires access to samples, rather than full token distributions.
% Sampled sequence distillation does not require access to the full token distribution, and removes the mismatch between data and soft labels--indeed, it captures the principled notion of distillation cross entropy. And, most 
% Importantly, we have precise control over what information is transferred, through what is \textit{sampled} from the teacher.
%\Skd works by applying constraints $c$ to this sampling:

%\begin{equation}
%    L_{SKD}(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim c(P_t)} logP_s(s)
%    \label{eq:seqCE}
%\end{equation}

%\noindent
% For instance, in our experiments, one aspect of constraint set $c$ is that we only sample knowledge related to specific notions of commonsense (verbalization \S\ref{sec:verbalization}). Another is that we constrain these samples to meet a learned notion of quality (purification \S\ref{sec:purification}). These ensure that, by the time the knowledge is distilled into a final model $P_s$ (\S\ref{sec:distillation}), it contains only the desired information. In a sense, we are not over-burdening student $P_s$ with learning irrelevant aspects of $P_t$ (GPT-3). This particular notion of distilling specific information from a general model, through text, is the central idea of \skd.

\subsection{Data: \atomicorig}
\label{subsec:atomicdata}

%As we describe \skd,
We demonstrate \skd on the \atomicorig \textit{if-then} resource \cite{sap2019atomic}.
%Our verablization (\S\ref{sec:verbalization}) and purificaiton (\S\ref{sec:purification}) result in a new \corpus--\autotomic. The distillation step produces a commonsense model--\model, much like past work using \atomicorig \cite{Bosselut2019COMETCT,hwang2020comet}. This past work provides state-of-the-art resources using using human-authored data--\atomic and \comet--to compare to our machine-generation. 
\atomicorig follows an event-relation-tail format. A large set of \textit{events} forms the foundation of the \corpus, e.g. \textit{X attacks Y}. An \atomicorig example links a relation to an event, like the \textbf{HinderedBy} relation which describes something that might hinder this event. For a given relation and head, the goal is to generate a resulting tail generation, e.g. \textit{X attacks Y} \textbf{HinderedBy} \textit{X is restrained}. 

Of the 23 relations from the most recent CSKB--\atomic--we limit our investigation to 7\footnote{We focus a subset of relations for simplicity of experimentation, and to test the limits of scale per-relation. By sampling many examples for a small number of relations, we can extrapolate our large-scale findings to unseen relations. With the same budget, we might generate fewer examples for more relations, yet not as closely understand the attributes of large per-relation scale.}: \textbf{xAttr} (how X is perceived after \textit{event}), \textbf{xReact} (how X reacts in response to \textit{event}), \textbf{xEffect} (what X does after \textit{event}), \textbf{xIntent} (X's intent in \textit{event}), \textbf{xWant} (what X wants after \textit{event}), \textbf{xNeed} (what X needed for \textit{event}) and \textbf{HinderedBy}. 

==> sections/backups/1_overview_4.tex <==
\section{Overview and Background}
\label{sec:overview}

Throughout our work, we describe the \textit{model--to--corpus--to--model} methodology of \skd, with model--to--corpus verbalization (\S\ref{sec:verbalization}), corpus--to--corpus purification (\S\ref{sec:purification}), and corpus--to--model distillation (\S\ref{sec:distillation}). Throughout, we contrast it with the best alternative \cite{hwang2020comet} that is authored by humans.

\Skd naturally follows the large--to--small model compression of knowledge distillation \citep{Hinton2015KnowledgeDistill}, yet our use of generated knowledge results in a fundamentally different process.

\subsection{Symbolic Knowledge Distillation}
\label{subsec:knowledgedistillation}

Our proposed methodology parallels knowledge distillation  \cite{Hinton2015KnowledgeDistill}, a method for
% The original motivation for KD was to
compressing a large or complicated teacher distribution $P_t$ into a smaller/simpler student distribution $P_s$. Key to knowledge distillation\footnote{In its simplest case, with temperature set to 1.0} is the notion of minimizing the cross-entropy between $P_t$ and $P_s$:

\begin{equation}
    H(P_t,P_s) = - \sum_{y \in Y} P_t(y) \log P_s(y)
    \label{eq:kd}
\end{equation}

\noindent
In effect, knowledge is transferred to the student by encouraging it to match predictions of the teacher. \citet{Hinton2015KnowledgeDistill} apply this to conditional classification: for each input example in a training set, $P_t$ and $P_s$ are model predictions over label set $Y$.

In our work, we would like to the distill knowledge from GPT-3, an unconditional language model--this will be $P_t$. This makes $Y$ the set of all strings, over which GPT-3 defines probability. This poses a problem for Eq~\ref{eq:kd}: summing over finite labels $Y$ was feasible, but summing over all infinite strings is not. 

Instead, we consider a sampling-based estimate of the same objective:

\begin{equation}
    L_{SKD}(P_t,P_s) = \mathop{\mathbb{E}}_{y \sim P^*_t(y)} [-\log P_{s}(y)]
\end{equation}

\noindent
With $P^*_t = P_t$, this is the same cross-entropy as Eq~\ref{eq:kd}, yet it can be estimated with finite samples from $P^*_t$--which come in the form of generations from GPT-3. Further, this allows fine-grained control over \emph{which} knowledge is distilled. We can set $P^*_t$ to truncated variants of GPT-3, for instance only those strings that cover a desired notion of commonsense (\S\ref{sec:verbalization}) with high quality (\S\ref{sec:purification}). This allows us to ensure, our distilled student model captures only the high-quality commonsense of teacher GPT-3 (\S\ref{sec:distillation}), rather than its full, general distribution.

% with as little performance degradation as possible. 
%In our work, the teacher is GPT-3 \cite{gpt3}, a 175-billion parameter language model.
% may be an ensemble of large speech recognition experts, whose knowledge is \textit{distilled} into a single student model $P_s$.
%, used here, is naturally a ``cumbersome'' model.

%both transfer knowledge from a large and ``cumbersome'' model to a compact and usable one. 

% While these methods optimize a similar objective, yet a key difference is \textit{generation} in \skd.

% This closely mirrors a section in the intro already.
% We devote 1 section to each of the 3 steps of \skd. First, \textit{model-to-\corpus}: we call this \textbf{verbalization} (\S\ref{sec:verbalization}). A large language model--GPT-3--\textit{generates} commonsense data; a large-scale generated CSKB is the result. Second, the \textbf{purification} step (\S\ref{sec:purification}), going \corpus-to-\corpus. Human evaluation tells us which generations are high quality; a discriminator trained on these human judgements does so as well, with surprising effectiveness. Here, we use this discriminator to filter down our CSKB, to high human-judged quality. Finally, going \textit{\corpus-to-model}, the \textbf{distillation} step (\S\ref{sec:distillation}). An efficient commonsense model is trained on our \corpus--the knowledge extracted from GPT-3. 
%\subsection{Knowledge Distillation by Generating}
%\label{subsec:knowledgedistillation}



%Knowledge distillation was introduced by \citet{Hinton2015KnowledgeDistill}, to transfer the learned knowledge from a ``cumbersome'' or

%Traditional knowledge distillation transfers knowledge to a student model $P_S$ by optimizing the student so that its outputs match those of a teacher $P_t$.
% parameters of $P_s$ 
% KD's training objective fixes the parameters of $P_t$, and optimizes $P_s$ 
% to match the teacher's outputs. 
%For language modeling, this means optimizing the parameters of $P_s$ to  minimize the cross entropy on each input sequence $x$:
% between a 
% For discrete distributions, this means minimizing the cross entropy between $P_t$ and $P_s$ for each input example $x$,
%\footnote{Softmax temperature $T=1$. Temperature is useful for controlling the learning signal but less principled in theory.},
% \begin{equation}
%     H(P_t,P_s,x) = -\sum_{v \in V} P_t(x)_v \log P_s(x)_v,
%     \label{eq:kd}
% \end{equation} 
% \noindent
% where $V$ is a vocabulary. % , such that the student model can \textit{author} commonsense.
% In language modeling, the distillation objective for a sequence $x$ is:
%$L(P_s;P_t,x) =$% Distil-GPT , given a 
% A natural way to do this is by introducing these soft labels to the language modelling objective for generation \footnote{distilGPT uses this method.}:
%\begin{equation}
%    -\sum_{i=1}^{|x|} \sum_{v \in V} P_t(x_i|x_{<i})_v\log P_s(x_{i}|x_{<i})_v.
%    \label{eq:Ldistilbert}
%\end{equation} 

%\noindent
%Instead of transferring knowledge via per-token probabilities, we are interested in transferring knowledge through natural language,
% . Natural language is a more appealing interface for our setting, 
% as it enables a controllable interface for knowledge curation, letting 
%as it enables us to edit, filter, and constrain the knowledge that is transferred. % (\S \ref{sec:purification}).
% , this enables ; and 2) we may not be interested in $P_s$ matching the distribution of $P_t$ for \emph{all} possible inputs --- for example, in this work, we are only interested in GPT-3's commonsense.
% (and not, say, it's \jack{something bad here like... IDK, dark reddit comments or something}).
%

%To this end, we develop a \textit{sampled sequence distillation} objective that operates on discrete sequences sampled from a constrained teacher $P_t^*$,
%\begin{equation}
%    L_{\mathrm{SKD}}(P_s; P_t) =  \mathop{\mathbb{E}}_{x \sim P^*_t(x)}[-\log P_s(x)].
%    \label{eq:seqCE}
%\end{equation}
%\noindent
%Operating on sequences enables knowledge transfer through natural language, while the constrained teacher $P_t^*$ -- formally, a distribution whose support is a subset of the original teacher's $P_t$ -- offers control over the transferred knowledge.
%For instance, an auxiliary model $A(x)$ can accept or reject sequences, $P^*_t(x) \propto P_t(x)\cdot A(x)$, which enables flexibly incorporating human feedback (\S\ref{sec:purification}).
%The objective corresponds to minimizing sequence-level cross-entropy, enabling controlled, natural language knowledge transfer in a principled way.

% we reformulate the language modeling KD objective (Eq~\ref{eq:Ldistilbert}) in two ways: 1) to enable a natural language interface, we operate on sampled sequences from $P_t$; and 2) we sample sequences $x$ from a constrained portion of the teacher distribution we are interested in reconstructing $P^*_t(x)$, rather than the full distribution $P_t(x)$. 
% The constraints we utilize are flexible. For example, prompt $p$ can specify the teacher distribution via $P^*_t(x) = P_t(x|p)$ (\S\ref{sec:verbalization}); and, an acceptability estimation model $A(x)$ an be directly for purification, i.e., $P^*_t(x) \propto P_t(x|p)\cdot A(x)$ (\S\ref{sec:purification}). For whichever curation is selected, for a constrained teacher $P^*_t(x)$, we optimize student using the \emph{sampled distillation} LM loss:

%Rather than distilling at the token level (Eq~\ref{eq:Ldistilbert}), we do this at the sequence level:
%In effect, replacing the gold word labels of the cross entropy with soft labels from $P_t$.
%However, in our work this is GPT-3, for which this distribution of soft labels is not currently available\footnote{At the time of writing, the API for GPT-3 only returns up to the top 100 token probabilities, out of thousands.}.
%There is also an intrinsic mismatch in this objective: the soft labels of $P_t$ come from a different distribution than the underlying data $x$.
%Most importantly, we do not want to distill \textit{all knowledge} from GPT-3 uniformly. GPT-3 contains a vast quantity of knowledge, and much is irrelevant--in this work we are only interested in its commonsense. We can imagine controlling this through the training data $x$ in Eq~\ref{eq:Ldistilbert}, yet we cannot control what is transferred through soft labels.

% \begin{equation}
%     L_{SKD}(P_t,P_s) =  \mathop{\mathbb{E}}_{x \sim P^*_t(x)}[-logP_s(x)]
%     \label{eq:seqCE}
% \end{equation}

% \noindent
% In effect, information about $P^*_t$ is captured by the frequentist notion of \textit{which full sequences $x$ it samples}, rather than soft word labels. 
% 
% \citet{Kim2016SequenceLevelKD} use a similar sequence-level formulation, but use only the mode from an unconstrained teacher.
% 
% rather than sample from distribution. 
% Operating on sequences enables knowledge transfer through natural language, and only requires access to samples, rather than full token distributions.
% Sampled sequence distillation does not require access to the full token distribution, and removes the mismatch between data and soft labels--indeed, it captures the principled notion of distillation cross entropy. And, most 
% Importantly, we have precise control over what information is transferred, through what is \textit{sampled} from the teacher.
%\Skd works by applying constraints $c$ to this sampling:

%\begin{equation}
%    L_{SKD}(P_t,P_s) =  lim_{n\xrightarrow{} \infty}\frac{1}{n}\sum_{s \sim c(P_t)} logP_s(s)
%    \label{eq:seqCE}
%\end{equation}

%\noindent
% For instance, in our experiments, one aspect of constraint set $c$ is that we only sample knowledge related to specific notions of commonsense (verbalization \S\ref{sec:verbalization}). Another is that we constrain these samples to meet a learned notion of quality (purification \S\ref{sec:purification}). These ensure that, by the time the knowledge is distilled into a final model $P_s$ (\S\ref{sec:distillation}), it contains only the desired information. In a sense, we are not over-burdening student $P_s$ with learning irrelevant aspects of $P_t$ (GPT-3). This particular notion of distilling specific information from a general model, through text, is the central idea of \skd.

\subsection{Data: \atomicorig}
\label{subsec:atomicdata}

%As we describe \skd,
We demonstrate \skd on the \atomicorig \textit{if-then} resource \cite{sap2019atomic}.
%Our verablization (\S\ref{sec:verbalization}) and purificaiton (\S\ref{sec:purification}) result in a new \corpus--\autotomic. The distillation step produces a commonsense model--\model, much like past work using \atomicorig \cite{Bosselut2019COMETCT,hwang2020comet}. This past work provides state-of-the-art resources using using human-authored data--\atomic and \comet--to compare to our machine-generation. 
\atomicorig follows an event-relation-tail format. A large set of \textit{events} forms the foundation of the \corpus, e.g. \textit{X attacks Y}. An \atomicorig example links a relation to an event, like the \textbf{HinderedBy} relation which describes something that might hinder this event. For a given relation and head, the goal is to generate a resulting tail generation, e.g. \textit{X attacks Y} \textbf{HinderedBy} \textit{X is restrained}. 

Of the 23 relations from the most recent commonsense knowledge graph--\atomic--we limit our investigation to 7 relations that correspond to \emph{causal} commonsense knowledge\footnote{We focus a subset of relations for simplicity of experimentation, and to test the limits of scale per-relation. By sampling many examples for a small number of relations, we can extrapolate our large-scale findings to unseen relations. With the same budget, we might generate fewer examples for more relations, yet not as closely understand the attributes of large per-relation scale.}: \textbf{xAttr} (how X is perceived after \textit{event}), \textbf{xReact} (how X reacts in response to \textit{event}), \textbf{xEffect} (what X does after \textit{event}), \textbf{xIntent} (X's intent in \textit{event}), \textbf{xWant} (what X wants after \textit{event}), \textbf{xNeed} (what X needed for \textit{event}) and \textbf{HinderedBy}. 

==> sections/backups/2_purification_0.tex <==
\section{Corpus-to-Corpus Purification}
\label{sec:purification}


Verbalization alone results in a viable CSKB. Indeed, the resulting corpus will already have advantages over human generated data: \autotomic has 10 times the scale of \atomic for the relations we test here. Yet, verbalization alone does not maximize the advantages of automatic generation; our much larger scale implies a much larger \emph{number of acceptable examples}. This will generally be true for automatically generated knowledge. Thus, we propose a second step, \textbf{purification}, to leverage the very large scale from verbalization to greatly increase CSKB accuracy. 

In this section, we describe the process of purification (\S\ref{subsec:purification}), and demonstrate its effect on the quality of \autotomic (\S\ref{subsec:purificationeval})

\subsection{Purifying a Generated CSKB}
\label{subsec:purification}

With a modest amount of supervision in the form of a small-scale human evaluation, we can train a model to predict and discriminate unacceptable examples--this is the idea of purification. Surprisingly, automatic models trained on human evaluation can discriminate unacceptable examples \emph{very effectively}, resulting in purified corpora that are both high quality and larger scale than human. Here, we describe this process, and its application to \autotomic.

\subsubsection{Human Supervision}

Purification requires human supervision, in the form of small-scale evaluation for tuning a model. We gather a training set of \textit{correct vs. incorrect} human judgments on a randomly-sampled set of 10K entries of \autotomic.  We follow the evaluation setup is in \S~\ref{subsec:atomichuman}, but gathering only one annotation for each example. We take a (random) train/dev/test split of 8k/1k/1k.

This aspect of \skd is not entirely automatic. Yet, we still avoid the complex task of human-authored knowledge. Evaluating 10k examples is both simpler and vastly cheaper than human construction of a corpus of equivalent scale (6.5 million examples).\footnote{To be the cost into perspective, our two acceptability evaluations (Table~\ref{tbl:ATOMIC-human}\&\ref{tbl:COMET-human}), which use 3 replicates, both require significantly more annotation than this set.} Instead, this should be viewed as a more useful and efficient role for humans in CSKB construction: evaluating a small number of examples at a high level.




\subsubsection{Purification Model}

To efficiently purify a CSKB, we train a classification model on the collected evaluation data, which can then be used to generate smaller and more accurate CSKBs by filtering. %We focus on general models with reasoning capabilities, which can be useful in future applications of \skd.

Specifically, we train binary classifiers for human acceptibility using RoBERTa-Large \cite{liu2019roberta}. We fine-tune all parameters, along with a 2-layer MLP on the \texttt{[CLF]} representation. We conduct a small grid search, finding batch size of 128, dropout of .1, and Adam \cite{kingma2014adam} learning rate of 5e-6. We use early stopping and decay learning rate on validation performance plateauing, to maximize $R@80\%$ on the validation set. We find RoBERTa pretrained on MNLI \cite{N18-1101} effective, substituting randomly-sampled names in for person designations ``X"/``Y".


%Specifically, we train binary classifiers for human acceptibility using RoBERTa-Large \cite{liu2019roberta}. We fine-tune all parameters, along with a 2-layer MLP on the \texttt{[CLF]} representation. We conduct a small grid search across batch size (\{64, \textbf{128}\}), dropout (\{\textbf{.1}, .4\}) and learning rate for Adam \cite{kingma2014adam} (1000 step linear warmup, \{5e-7, 1e-6, \textbf{5e-6}\}); we use early stopping and decay learning rate on validation performance plateauing, in an effort to maximize $R@80\%$ on the validation set. We find that RoBERTa pretrained on MNLI \cite{N18-1101} effective, substituting randomly-sampled names in for person designations ``X"/``Y".

For corpus filtering, we include an unsupervised filtration metric inspired by \cite{davison2019commonsense} as a baseline: they propose using a model estimate of PMI to score mined KB triples. In our case, we use the Negative Log-Likelihood (NLL) and token-mean-NLL from GPT-3 itself. %The intuition is that the model-estimated generation probabilities may already carry some information about validity.

The validation precision/recall of our best performing model, the baseline, and the in-optimal hyperparameter configurations we tried are given in Figure~\ref{fig:prec-v-rec}. Finally, we applied the best model to the test set (also in Fig~\ref{fig:prec-v-rec}), verifying that it generalizes to \autotomic entries.

Overall, our trained purification model is very effective: the classifier results in a higher precision corpus than many extracted+human authored KBs at reasonable recall levels, e.g., keeping 60\% of correct \autotomic generations, the resulting precision is 95\%. In comparison, using GPT-3's NLL cutoff directly is not competitive. As a result of our experiments, we suggest RoBERTa-Large pretrained on MNLI as a starting point for the purification step, with our stated hyperparameters. %Using this model with our stated hyperparameters results in very high accuracy while retaining scale, e.g. accuracy of 96.4\% while keeping over a third of the generated data. 


\input{figures/pre_v_rec}

\subsection{The Effect of Purification}
\label{subsec:purificationeval}

\paragraph{Does Human Acceptability Improve?}
The goal of purification is raising the quality of our generated corpus, \autotomic. By human evaluation (Table~\ref{tbl:COMET-human}--\S\ref{subsec:verbalization-eval}) we can see that this is successful. The top row of \autotomic--without purification--has a human acceptance rate of 78.5\%. Even under our lowest threshold for purification (second row of), this rises to 88.4\% acceptance, exceeding the human-generated \atomic. Our highest setting increases this to 96.4\, a full 17.9 points above the unpurified corpus. Indeed, a small amount of human supervisions results in a highly effective purifier.

\paragraph{Size-accuracy Trade-off?}
Naturally, there is a trade-off between size and accuracy in \autotomic--purification works by filtering data points, resulting in a smaller corpus. Yet comparing to human-generated \atomic tells us the trade-off is favorable. By reducing size from 6.5M to 5.1M (approx. 20\% reduction), the \autotomic can already surpass the accuracy of \atomic. Reducing to 2.5M examples (38\% of the original size), we can attain an accuracy of 96.4\%, nearly 10 points above the human corpus. To put this in perspective, at this level of purification \autotomic is still 4X larger than \atomic. One takeaway is that scale is a strong advantage of automatic knowledge generation: attempting a similar filtering step on human-generated \atomic would further reduce its already smaller size. 

\paragraph{What gets filtered out?}

\paragraph{Changes to Diversity?}

Besides raising accuracy, how does purification affect \autotomic? One attribute we are particularly interested in diversity--one could imagine purification reducing \autotomic to only very similar examples or ``safe bets'' that might not be useful in practice. To test this, we extend our diversity analysis from \S\ref{subsec:verbalization-eval} in Table~\ref{tbl:ATOMIC-diverse-ex}, measuring the number of lexically novel examples as the corpus is purified. Naturally, as we filter examples, we are filtering some \emph{diverse} examples. This gives no indication that the relative diversity of the corpus goes down: \autotomic at its full size is made up of about 68\% \emph{diverse} examples, and at its most purified this actually goes up to 80\%. 

Yet diversity and human-judged quality do not tell the whole story. We are not only interested in these intrinsic measures--we are interested in whether or not a generated CSKB will be \textit{useful} in practice. To study this, we move onto distillation \S\ref{sec:distillation}, where we measure how useful each corpus is for training a downstream commonsense model. 

==> sections/backups/abstract_0.tex <==
\begin{abstract}

In the past, commonsense knowledge has gone \textit{human-to-corpus-to-model}: humans author commonsense knowledge bases (CSKBs), which are used to train commonsense models. We present an alternative, \textit{model-to-corpus-to-model}: large and general models \emph{generate} the CSKB on which commonsense models are trained. We call our method \textbf{\skd}, taking inspiration from knowledge distillation, in which large models teach smaller models.

Yet, we differ from much work on knowledge distillation in one key point: our distilled model \emph{exceeds} the teacher--GPT-3--despite its smaller size. %Generating \atomicorig \textit{if-then} data, we find our commonsense model--trained on generated data--exceeds the generator by 8 points.
Another difference is that we represent the distilled knowledge explicitly--the generated CSKB, which is a natural produce of our method. Explicitly generating knowledge allows us to control what is distilled, \textit{only the commonsense} of the large general model; we can also purify that knowledge by filtering. With purification, we outperform the \textit{human-to-corpus-to-model} paradigm: our generated corpus exceeds the quality and scale of the human-authored corpus, and results in a superior commonsense model to the human-authored knowledge (by 9.6 and 6 accuracy points, respectively).

We apply \skd to the \atomicorig resource, resulting in a new CSKB (\autotomic) and commonsense model (\model), both exceeding past work. \Skd presents a new paradigm for commonsense research--in which humans need not be the only source for high-quality knowledge.

\end{abstract}

==> sections/backups/abstract_2.tex <==
\begin{abstract}
Past efforts to endow agents with commonsense knowledge follow a human-to-\corpus-to-model paradigm, in which humans author commonsense knowledge bases that are used to train downstream models.
We depart from this approach, and present \textbf{\skd}: a methodology which uses a large-scale language model -- rather than humans -- to author common-sense knowledge that is purified based on human feedback and used to train efficient commonsense models.
We use symbolic knowledge distillation along with GPT-3 to create a corpus based on the human-authored \atomicorig knowledge base, at a fraction of its cost, while being an order of magnitude larger and of higher quality.
Downstream models are more effective than those trained on the human-authored corpus, and are smaller, yet more powerful, than the teacher model.
Symbolic knowledge distillation shifts human effort from authoring knowledge to providing feedback, presenting a new  model-to-corpus-to-model paradigm for commonsense research, in which machines complement humans as sources of high-quality knowledge.
\end{abstract}

==> sections/backups/abstract_3_jack.tex <==
\begin{abstract}

In the past, commonsense knowledge has been transferred from \textit{human-to-\corpus-to-model}: \peter{or \textit{human-to-CSKB-to-model}? if so, change the macro} humans author commonsense knowledge bases (CSKBs), which are used to train commonsense models. We present an alternative, \textit{model-to-\corpus-to-model}: large and general models first \emph{generate} the CSKB on which commonsense models are subsequently trained. We call our method \textbf{\skd}: taking inspiration from knowledge distillation, in which large models teach smaller models.
%Generating \atomicorig \textit{if-then} data, we find our commonsense model--trained on generated data--exceeds the generator by 8 points.
%Our method outperforms prior work primarily because of a purification step;

Because the teacher's intermediate representation is a human-readable KB
(instead of logits, as in standard distillation), \skd
enables
%which is a natural produce of our method.
curation on what information is transferred to the student, e.g., logically inconsistent entries can be removed.
%\textit{only the commonsense} of the large general model.
%Textual knowledge can also be purified, by filtering.
%With a purification step, \skd outperforms the \textit{human-to-\corpus-to-model} paradigm:
With such a purification step,
%Yet, we differ from much work on knowledge distillation in that
our distilled model \emph{exceeds} the performance of the teacher (here, GPT-3) despite its 100x smaller size. And, when applied to the  \atomicorig resource, our generated \corpus exceeds the quality and scale of the human-authored \corpus, and results in a superior commonsense model (by 9.6 and 6 accuracy points, respectively).
\Skd presents a new paradigm for commonsense research--in which humans need not be the only source for high-quality knowledge.

%We apply \skd to the \atomicorig resource, resulting in a new CSKB and commonsense model--\textbf{\autotomic} and \textbf{\model}--both exceeding past work.

%%%%%%
%%%% Old abstract: 
%%%%%%

%In the past, commonsense knowledge has gone \textit{human-to-\corpus-to-model}: \peter{or \textit{human-to-CSKB-to-model}? if so, change the macro} humans author commonsense knowledge bases (CSKBs), which are used to train commonsense models. We present an alternative, \textit{model-to-\corpus-to-model}: large and general models \emph{generate} the CSKB on which commonsense models are trained. We call our method \textbf{\skd}, taking inspiration from knowledge distillation, in which large models teach smaller models.

%Yet, we differ from much work on knowledge distillation in one key point: our distilled model \emph{exceeds} the teacher--GPT-3--despite its smaller size.
%Another difference is that we represent the distilled knowledge explicitly--the generated CSKB, which is a natural produce of our method. Explicitly generating knowledge allows us to control what is distilled, \textit{only the commonsense} of the large general model. Textual knowledge can also be purified, by filtering. With purification, we outperform the \textit{human-to-\corpus-to-model} paradigm: our generated \corpus exceeds the quality and scale of the human-authored \corpus, and results in a superior commonsense model to the human-authored knowledge (by 9.6 and 6 accuracy points, respectively).

%We apply \skd to the \atomicorig resource, resulting in a new CSKB and commonsense model--\textbf{\autotomic} and \textbf{\model}--both exceeding past work. \Skd presents a new paradigm for commonsense research--in which humans need not be the only source for high-quality knowledge.



\end{abstract}

==> tables/automic_examples.tex <==
% \begin{table*}[!t]
% % \footnotesize
% % \small
% \setlength{\tabcolsep}{4pt}
% \begin{center}
% \begin{tabular}{l}
% \toprule
% Head, \textbf{Relation}, Tail \\

% \midrule

% % X escapes from the cage & \texttt{HinderedBy} & X is in a coma \\
% % % X decides to look on the bright side & \texttt{xNeed} & to decide to be optimistic \\
% % X imagines some outrageous plans & \texttt{xNeed} & to have a crazy imagination \\
% % X considers the inheritance & \texttt{xWant} & to see the will \\
% % X changes his travel plans & \texttt{xIntent} & to visit a new place \\
% % X finds a free babysitter & \texttt{xReact} & delighted \\
% % X charges a service fee & \texttt{xAttr} & professional \\
% % X gets a good idea & \texttt{xEffect} & is congratulated by his boss \\

% X escapes from the cage \textbf{is hindered by} X is in a coma. \\
% X imagines some outrageous plans. \textbf{Before, X needs} to have a crazy imagination. \\
% X considers the inheritance. \textbf{As a result, X wants} to see the will. \\
% X changes his travel plans. \textbf{Before, X wanted} to visit a new place. \\
% X finds a free babysitter. \textbf{As a result, X feels} delighted. \\
% X charges a service fee. \textbf{As a result, X is seen as} professional. \\
% X gets a good idea. As a result, X is congratulated by his boss. \\


% \bottomrule
% \end{tabular}
% \end{center}
% \caption{
% \automic examples
% }
% \label{tbl:AUTOMIC-examples}
% \end{table*}


% \begin{table}[!t]
% % \footnotesize
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{center}
% \begin{tabular}{ll}
% \toprule
% % Head, \textbf{Relation}, Tail \\

% % \midrule

% % X escapes from the cage & \texttt{HinderedBy} & X is in a coma \\
% % % X decides to look on the bright side & \texttt{xNeed} & to decide to be optimistic \\
% % X imagines some outrageous plans & \texttt{xNeed} & to have a crazy imagination \\
% % X considers the inheritance & \texttt{xWant} & to see the will \\
% % X changes his travel plans & \texttt{xIntent} & to visit a new place \\
% % X finds a free babysitter & \texttt{xReact} & delighted \\
% % X charges a service fee & \texttt{xAttr} & professional \\
% % X gets a good idea & \texttt{xEffect} & is congratulated by his boss \\

% X escapes from the cage \\
% \textbf{is hindered by} X is in a coma. \\
% \midrule

% X imagines some outrageous plans. \\
% \textbf{Before, X needs} to have a crazy imagination. \\
% \midrule

% X considers the inheritance. \\
% \textbf{As a result, X wants} to see the will. \\
% \midrule

% X changes his travel plans. \\ 
% \textbf{Before, X wanted} to visit a new place. \\
% \midrule

% X finds a free babysitter. \\
% \textbf{As a result, X feels} delighted. \\
% \midrule

% X charges a service fee. \\
% \textbf{As a result, X is seen as} professional. \\
% \midrule
% X gets a good idea. \\
% \textbf{As a result, X} is congratulated by his boss. \\

% \bottomrule
% \end{tabular}
% \end{center}
% \caption{
% \automic examples
% }
% \label{tbl:AUTOMIC-examples}
% \end{table}


\begin{table}[!t]
% \footnotesize
\small
\setlength{\tabcolsep}{4pt}
\begin{center}
\begin{tabular}{l|l}
\toprule
% Head, \textbf{Relation}, Tail \\

% \midrule

% X escapes from the cage & \texttt{HinderedBy} & X is in a coma \\
% % X decides to look on the bright side & \texttt{xNeed} & to decide to be optimistic \\
% X imagines some outrageous plans & \texttt{xNeed} & to have a crazy imagination \\
% X considers the inheritance & \texttt{xWant} & to see the will \\
% X changes his travel plans & \texttt{xIntent} & to visit a new place \\
% X finds a free babysitter & \texttt{xReact} & delighted \\
% X charges a service fee & \texttt{xAttr} & professional \\
% X gets a good idea & \texttt{xEffect} & is congratulated by his boss \\

Head & X escapes from the cage \\
Rel+Tail & \textbf{is hindered by} X is in a coma. \\
\midrule

Head & X imagines some outrageous plans. \\
Rel+Tail & \textbf{Before, X needs} to have a crazy imagination. \\
\midrule

Head & X considers the inheritance. \\
Rel+Tail & \textbf{As a result, X wants} to see the will. \\
\midrule

Head & X changes his travel plans. \\ 
Rel+Tail & \textbf{Before, X wanted} to visit a new place. \\
\midrule

Head & X finds a free babysitter. \\
Rel+Tail & \textbf{As a result, X feels} delighted. \\
\midrule

Head & X charges a service fee. \\
Rel+Tail & \textbf{As a result, X is seen as} professional. \\
\midrule
Head & X gets a good idea. \\
Rel+Tail & \textbf{As a result, X} is congratulated by his boss. \\

\bottomrule
\end{tabular}
\end{center}
\caption{
GPT-3 generated \automic examples
}
\label{tbl:AUTOMIC-examples}
\end{table}

==> tables/backups/tbl_tail_tokens_by_relation.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{4pt}
\begin{center}
\footnotesize
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Length}} & \multicolumn{2}{c}{\textbf{Unique Tokens}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textbf{\atomic} & \textbf{\automic} & \textbf{\atomic} & \textbf{\automic}\\
\texttt{xWant} & 4.69 & 5.16 & 322K & 784K \\
\texttt{xAttr} & 1.42 & 2.73 & 15K & 21K \\
\texttt{xEffect} & 3.92 & 4.66 & 216K & 864K \\
\texttt{xIntent} & 4.59 & 5.92 & 136K & 800K \\
\texttt{xNeed} & 4.51 & 5.97 & 289K & 1,378K \\
\texttt{xReact} & 4.03 & 1.77 & 48K & 5K \\
\texttt{HinderedBy} & 7.93 & 7.49 & 522K & 1,775K \\ 
\midrule
Heads & 5.20 & 5.32 & 109K & 881K\\
\bottomrule
\end{tabular}
\end{center}
\caption{
Average length and total unique tokens in tails by relation type, and in heads (bottom row) from \atomic\ and \automic.
Head statistics are reported once for all relations since they remain essentially constant across all relations.
}
\label{tbl:tail-tokens-by-relation}
\end{table}

==> tables/comet_gen_examples.tex <==
\begin{table}[!t]
% \footnotesize
\small
\setlength{\tabcolsep}{4pt}
\begin{center}
\begin{tabular}{l|llc}
\toprule
Head+Rel & Model & Tail & Judge \\

\midrule

 \multirow{4}{*}{\makecell[tl]{X asks Y \\ to sit \\ \\\textbf{\textit{xAttr}}}} & \cometshort & curious & \xmark \\
 & \model & polite & \cmark \\
 & \ $+\text{pure}_\text{low}$ & polite & \cmark \\
 & \ $+\text{pure}_\text{high}$& polite & \cmark \\
 
 \midrule
 
  \multirow{4}{*}{\makecell[tl]{X packs \\ my bags \\ \\\textbf{\textit{xNeed}}}} & \cometshort & nothing in particular & \xmark \\
 & \model & to pack my bags & \xmark \\
 & \ $+\text{pure}_\text{low}$& to be in charge of packing & \cmark \\
 & \ $+\text{pure}_\text{hi}$ & to be moving out & \cmark \\
 
 \midrule
 
  \multirow{4}{*}{\makecell[tl]{X flees the \\ scene \\ \\\textbf{\textit{xReact}}}} & \cometshort & relieved & \cmark \\
 & \model & guilty & \cmark \\
 & \ $+\text{pure}_\text{low}$ & ashamed & \cmark \\
 & \ $+\text{pure}_\text{high}$ & ashamed & \cmark \\

 
\bottomrule
\end{tabular}
\end{center}
\caption{
Tail generations from \comet and \model, trained on full \autotomic (\model), and \autotomic purified to 82.9\% and 96.4\%.
}
\label{tbl:COMET-examples}
\end{table}


==> tables/purify_ablation_0.tex <==
\begin{table}[]
\begin{center}
%\resizebox{\linewidth}{!}{
%    \begin{tabular}{c|cccccc}
%    \toprule
%           & $f_o$ & $f(h)$  & $f(t)$  & $f_1(h)+f_2(t)$ & $EMAP(f(h,t))$ & $f(h,t)$\\
%           \midrule
%        AP & 79  & 86 & 82 & 86 &   87  & \textbf{94} \\
%        \bottomrule
%    \end{tabular}
%}
\begin{tabular}{l | c}
\toprule
& AP \\
\midrule
Random & 79.3 \\
Inference-only & 81.9 \\
Event-only & 86.2 \\
EMAP(Full model) &  87.1\\
Full model & \textbf{94.0}\\
\bottomrule
\end{tabular}
\end{center}
\caption{Average Precision for ablations of the critic model (higher=better). The critic model not only filters out \emph{awkward phrasings} (which can be identified looking at either the event or inference in isolation: EMAP can only identify these), but also filters out \emph{logical misalignments}, which require modeling interactions between the event/inference. %\liwei{Event-only, Inference-only?}
}
\label{tbl:purification_ablation}
\end{table}

% AP of different models. we will throw relation in with head only so head only model is really head, relation (arbitrary).
%Random 0.793287895959581
%results~model=roberta-large-mnli~flatten=relation_only~lr=5e-06~bs=128~dropout=0.10.json 0.8076747160231097
%results~model=roberta-large-mnli~flatten=head_and_relation_only~lr=5e-06~bs=128~dropout=0.10.json 0.8619407141183499
%results~model=roberta-large-mnli~flatten=C~lr=5e-06~bs=128~dropout=0.10.json 0.9401695562327921
%results~model=roberta-large-mnli~flatten=head_and_tail_only~lr=5e-06~bs=128~dropout=0.10.json 0.9106221581481693
%results~model=roberta-large-mnli~flatten=head_only~lr=5e-06~bs=128~dropout=0.10.json 0.8558616238056735
%results~model=roberta-large-mnli~flatten=tail_only~lr=5e-06~bs=128~dropout=0.10.json 0.8191037234118135
%results~model=roberta-large-mnli~flatten=tail_and_relation_only~lr=5e-06~bs=128~dropout=0.10.json 0.8334948065728878
% ENSEMBLE AP = 86.28

% EMAP ALL:
% Orig AUC: 81.12
%random AUC: 49.24046617636692
%ensemble of head-only and tail-only, additively (EMAP) AUC: 63.25
%head-only AUC: 64.07
%tail-only AUC: 56.60
%Orig AP: 93.99
% same as above, good check.
%random AP: 79.3287895959581
%ensemble of head-only and tail-only, additively (EMAP) AP: 87.08
%head-only AP: 87.54
%tail-only AP: 83.10


==> tables/tbl_all_size_stats.tex <==
\begin{table}
\footnotesize
\begin{tabular}{llrrrrrrrr}
\toprule
    &relation &  unique\_heads\_autotomic &  unique\_heads\_atomic &  unique\_tails\_autotomic &  unique\_tails\_atomic &  unique\_triples\_autotomic &  unique\_triples\_atomic &  triples\_autotomic &  triples\_atomic \\
\midrule
& HinderedBy &                  165783 &                11024 &                  237169 &                65847 &                   1028092 &                  77616 &            1657830 &           77616 \\
1 &       xNeed &                  165783 &                20836 &                  230902 &                64029 &                    760232 &                 100995 &            1657830 &          105557 \\
2 &       xWant &                  165783 &                20300 &                  152004 &                68594 &                    730223 &                 109098 &            1657830 &          110009 \\
3 &     xIntent &                  165783 &                20629 &                  135215 &                29621 &                    965921 &                  54839 &            1657830 &           58997 \\
4 &      xReact &                  165783 &                20353 &                    2751 &                11796 &                   1033123 &                  62424 &            1657828 &           65984 \\
5 &       xAttr &                  165783 &                20388 &                    7704 &                10532 &                    884318 &                 113096 &            1657145 &          120447 \\
6 &     xEffect &                  165783 &                20391 &                  185358 &                55176 &                   1054391 &                  90868 &            1657829 &           93413 \\
7 &         All &                  165783 &                21006 &                  874417 &               289536 &                   6456300 &                 608936 &           11604122 &          632023 \\
\bottomrule
\end{tabular}
\caption{}
\label{tbl:size-stats-full}
\end{table}

==> tables/tbl_head_tail_tokens_aggregate.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{4pt}
\begin{center}
\footnotesize
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Heads}} & \multicolumn{2}{c}{\textbf{Tails}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textbf{Length} & \textbf{Uniq-tok} & \textbf{Length} & \textbf{Uniq-tok}\\
 \atomic & 5.20 & 109k & 5.18 & 1.5m\\
 \automic& 5.32 & 881k & 6.02 & 5.2m\\
\bottomrule
\end{tabular}
\end{center}
\caption{
Average length and total unique tokens in heads and tails from \automic\ and \atomic.
}
\label{tbl:head-tail-tokens-aggregate}
\end{table}

==> tables/tbl_self_bleu.tex <==
\begin{table}[!t]
\setlength{\tabcolsep}{4pt}
\begin{center}
\footnotesize
\begin{tabular}{l|c|cc}
\toprule
\textbf{Corpus}   & Accuracy & Size & Diverse Examples\\
\midrule
\atomic             & 86.8 &   0.61M  &  0.56M \\
\midrule
\autotomic{} &  78.5 &  6.46M & 4.38M \\
 &    88.4 &   5.10M & 3.68M\\
 &    91.5 &    4.40M & 3.25M\\
 &    94.3 &    3.62M & 2.74M\\
 &    95.3 &    3.02M & 2.33M\\
 &    96.4 & 2.51M & 2.00M\\

\bottomrule
\end{tabular}
\end{center}
\caption{The number of diverse examples in each corpus, defined as the number of \emph{softly unique} points as defined in \S\ref{subsec:verbalization-eval}. Besides being larger, \autotomic corpora also contain more diverse examples than \atomic.}
\label{tbl:ATOMIC-diverse-ex}
\end{table}

% \footnote doesn't work in caption, need to just mark then put the footnote below
\footnotetext{Size of \atomic is given as the number of comparable datapoints, i.e. those with the same relations as \autotomic{}.}

